Latent Task-Specific Graph Network Simulators

Simulating dynamic physical interactions is a critical challenge across multiple scientific domains, with applications ranging from robotics to material science. For mesh-based simulations, Graph Network Simulators (GNSs) pose an efficient alternative to traditional physics-based simulators. Their inherent differentiability and speed make them particularly well-suited for inverse design problems. Yet, adapting to new tasks from limited available data is an important aspect for real-world applications that current methods struggle with. We frame mesh-based simulation as a meta-learning problem and use a recent Bayesian meta-learning method to improve GNSs adaptability to new scenarios by leveraging context data and handling uncertainties. Our approach, latent task-specific graph network simulator, uses non-amortized task posterior approximations to sample latent descriptions of unknown system properties. Additionally, we leverage movement primitives for efficient full trajectory prediction, effectively addressing the issue of accumulating errors encountered by previous auto-regressive methods. We validate the effectiveness of our approach through various experiments, performing on par with or better than established baseline methods. Movement primitives further allow us to accommodate various types of context data, as demonstrated through the utilization of point clouds during inference. By combining GNSs with meta-learning, we bring them closer to real-world applicability, particularly in scenarios with smaller datasets.

==> main/3_foundations.tex <==
% \section{Foundations}
% \gpt{
% Graph Network Simulators (GNSs) represent a significant advancement in the field of simulating complex physical interactions. These simulators are designed to model systems as graphs, where nodes represent entities, and edges capture their relationships. This foundational section aims to elucidate key principles of GNSs.
% In GNSs, the physical system under consideration is often translated into a graph representation, denoted as $G = (V, E)$, where 
% $V$ represents nodes corresponding to entities within the system, and $E$ signifies edges capturing pairwise interactions.
% Central to GNSs is the concept of Message Passing Networks (MPNs), where information exchange occurs between neighboring nodes within the graph. This iterative message passing process leverages collective knowledge to capture complex interactions.
% Graph Neural Networks (GNNs), a specific class of GNSs, implement message passing using neural networks. GNNs update node representations by aggregating information from neighboring nodes, facilitating hierarchical feature learning. The node update process in GNNs involves weighted summation of neighboring node features and activation functions.
% This foundational understanding of GNSs, emphasizing graph representations and message passing, forms the basis for their application in simulating intricate physical systems.
% }
% \subsection{Gaussian Mixture Model Neural Processes}
% \paragraph{Non-amortized meta-learning}
% \paragraph{Task specification through optimization, e.g. GradientVIPS}



==> main/6_results.tex <==
\textbf{Results}
\input{main/figure_wrappers/04_figure_bar_plots}
Here, we show how good \gls{ltsgns} is.






